Blocking Underhand Attacks by Hidden Coalitions (Extended Version)

Similar to what happens between humans in the real world, in open multi-agent systems distributed over the Internet, such as online social networks or wiki technologies, agents often form coalitions by agreeing to act as a whole in order to achieve certain common goals. However, agent coalitions are not always a desirable feature of a system, as malicious or corrupt agents may collaborate in order to subvert or attack the system. In this paper, we consider the problem of hidden coalitions, whose existence and the purposes they aim to achieve are not known to the system, and which carry out so-called underhand attacks. We give a first approach to hidden coalitions by introducing a deterministic method that blocks the actions of potentially dangerous agents, i.e. possibly belonging to such coalitions. We also give a non-deterministic version of this method that blocks the smallest set of potentially dangerous agents. We calculate the computational cost of our two blocking methods, and prove their soundness and completeness.

==> abstract.tex <==
\fontsize{9}{11}\selectfont Similar to what happens between humans in
the real world, in open multi-agent systems distributed over the
Internet, such as online social networks or wiki technologies, agents
often form coalitions by agreeing to act as a whole in order to achieve
certain common goals. However, agent coalitions are not always a
desirable feature of a system, as malicious or corrupt agents may
collaborate in order to subvert or attack the system. In this paper, we
consider the problem of hidden coalitions, whose existence and the
purposes they aim to achieve are not known to the system, and which
carry out so-called underhand attacks. We give a first approach to
hidden coalitions by introducing a deterministic method that blocks the
actions of potentially dangerous agents, i.e. possibly belonging to such
coalitions. We also give a non-deterministic version of this method that
blocks the smallest set of potentially dangerous agents. We calculate
the computational cost of our two blocking methods, and prove their
soundness and completeness.


==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
  Matteo Cristani, Erisa Karafili, Luca Vigan\`o\\
  \fontsize{9}{11}\selectfont
  \textit{Dipartimento di Informatica, Universit\`a degli Studi di Verona, Italy}\\
  \fontsize{9}{11}\selectfont
  \textit{\{matteo.cristani,erisa.karafili,luca.vigano\}@univr.it}
\\[12pt]
}


==> keywords.tex <==
\fontsize{9}{11}\selectfont Multi-agent systems, coalitions, security, blocking attacks.


==> title.tex <==
% The Title is all in Uppercase
\newcommand{\mytitle}{\uppercase{Blocking Underhand Attacks By Hidden Coalitions (Extended Version)}
}

